What Does an Observability Foundation Model Know?

A linear probe can show that a label is recoverable from a model's hidden states, but not whether that goes beyond what the input already reveals, or whether the model uses it. We audit Toto, an observability forecasting foundation model, on the Benchmark of Observability Metrics (BOOM) across five series-disjoint resplits, comparing linear probes on its frozen residual stream with models that read the raw input window and with Toto's architecture stripped of its trained configuration. Short-vs-medium cadence and metric type are more linearly recoverable from Toto's residuals than from the strongest raw-window model in every resplit (macro-F1 0.766 vs. 0.633 and 0.545 vs. 0.498). Domain is nearly tied, and series cardinality is recovered far better from the raw window. MOMENT-base shows related cadence, metric-type, and domain readouts. Recoverability is not use: exchanging Toto's residuals with those of high-burst donors moves a future-burstiness readout as intended but does not make forecasts consistently burstier than a randomized donor. A BOOM-trained coordination probe has negative zero-shot R^2 on the tested external benchmarks. We report each label against its strongest baseline.

==> figures/tikz/gen/fig1_panel1.tex <==
\draw[fig1 ref] (axis cs:0.766055,0.4) -- (axis cs:0.766055,6.6);
\addplot[fig1 toto] coordinates {(0.766055,6) +- (0.024369,0)};
\addplot[fig1 raw] coordinates {(0.633490,5) +- (0.047014,0)};
\addplot[fig1 control] coordinates {(0.566733,4) +- (0.019787,0)};
\addplot[fig1 control] coordinates {(0.547446,3) +- (0.040006,0)};
\addplot[fig1 control] coordinates {(0.408811,2) +- (0.047152,0)};
\addplot[fig1 control] coordinates {(0.485754,1) +- (0.011448,0)};
\node[fig1 fam, anchor=east] at (axis cs:0.5715,5) {FNO};


==> figures/tikz/gen/fig1_panel2.tex <==
\draw[fig1 ref] (axis cs:0.545326,0.4) -- (axis cs:0.545326,6.6);
\addplot[fig1 toto] coordinates {(0.545326,6) +- (0.037481,0)};
\addplot[fig1 raw] coordinates {(0.497942,5) +- (0.007220,0)};
\addplot[fig1 control] coordinates {(0.419774,4) +- (0.016109,0)};
\addplot[fig1 control] coordinates {(0.397733,3) +- (0.034538,0)};
\addplot[fig1 control] coordinates {(0.347452,2) +- (0.029673,0)};
\addplot[fig1 control] coordinates {(0.321383,1) +- (0.032037,0)};
\node[fig1 fam, anchor=east] at (axis cs:0.4757,5) {GBDT};


==> figures/tikz/gen/fig1_panel3.tex <==
\draw[fig1 ref] (axis cs:0.484078,0.4) -- (axis cs:0.484078,6.6);
\addplot[fig1 toto] coordinates {(0.484078,6) +- (0.011356,0)};
\addplot[fig1 raw] coordinates {(0.482457,5) +- (0.040245,0)};
\addplot[fig1 control] coordinates {(0.394373,4) +- (0.011024,0)};
\addplot[fig1 control] coordinates {(0.362205,3) +- (0.016629,0)};
\addplot[fig1 control] coordinates {(0.371480,2) +- (0.037414,0)};
\addplot[fig1 control] coordinates {(0.317341,1) +- (0.036506,0)};
\node[fig1 fam, anchor=east] at (axis cs:0.4272,5) {GBDT};


==> figures/tikz/gen/fig1_panel4.tex <==
\draw[fig1 ref] (axis cs:0.471399,0.4) -- (axis cs:0.471399,6.6);
\addplot[fig1 toto] coordinates {(0.471399,6) +- (0.029233,0)};
\addplot[fig1 raw] coordinates {(0.960976,5) +- (0.015733,0)};
\addplot[fig1 control] coordinates {(0.428168,4) +- (0.127259,0)};
\addplot[fig1 control] coordinates {(0.250479,3) +- (0.025485,0)};
\addplot[fig1 control] coordinates {(0.635367,2) +- (0.027198,0)};
\addplot[fig1 control] coordinates {(0.216750,1) +- (0.028967,0)};
\node[fig1 fam, anchor=east] at (axis cs:0.9302,5) {FNO};


==> figures/tikz/gen/fig3_defs.tex <==
\def\figThreeFamA{FNO}\def\figThreeWinsA{5}
\def\figThreeFamB{GBDT}\def\figThreeWinsB{5}
\def\figThreeFamC{GBDT}\def\figThreeWinsC{2}
\def\figThreeFamD{FNO}\def\figThreeWinsD{0}


==> figures/tikz/gen/fig3_panel1.tex <==
\addplot[fig3 up] coordinates {(0,0.742072) (1,0.689504)};
\addplot[fig3 up] coordinates {(0,0.768100) (1,0.618053)};
\addplot[fig3 up] coordinates {(0,0.788583) (1,0.597782)};
\addplot[fig3 up] coordinates {(0,0.780820) (1,0.654205)};
\addplot[fig3 up] coordinates {(0,0.750698) (1,0.607906)};
\addplot[fig3 mean] coordinates {(0,0.766055) (1,0.633490)};


==> figures/tikz/gen/fig3_panel2.tex <==
\addplot[fig3 up] coordinates {(0,0.501100) (1,0.493516)};
\addplot[fig3 up] coordinates {(0,0.584081) (1,0.499838)};
\addplot[fig3 up] coordinates {(0,0.544186) (1,0.494660)};
\addplot[fig3 up] coordinates {(0,0.557678) (1,0.494351)};
\addplot[fig3 up] coordinates {(0,0.539584) (1,0.507344)};
\addplot[fig3 mean] coordinates {(0,0.545326) (1,0.497942)};


==> figures/tikz/gen/fig3_panel3.tex <==
\addplot[fig3 up] coordinates {(0,0.490268) (1,0.433633)};
\addplot[fig3 down] coordinates {(0,0.490715) (1,0.515278)};
\addplot[fig3 up] coordinates {(0,0.469650) (1,0.467565)};
\addplot[fig3 down] coordinates {(0,0.480255) (1,0.493315)};
\addplot[fig3 down] coordinates {(0,0.489505) (1,0.502493)};
\addplot[fig3 mean] coordinates {(0,0.484078) (1,0.482457)};


==> figures/tikz/gen/fig3_panel4.tex <==
\addplot[fig3 down] coordinates {(0,0.452960) (1,0.964409)};
\addplot[fig3 down] coordinates {(0,0.502992) (1,0.947869)};
\addplot[fig3 down] coordinates {(0,0.468751) (1,0.955310)};
\addplot[fig3 down] coordinates {(0,0.445937) (1,0.981072)};
\addplot[fig3 down] coordinates {(0,0.486356) (1,0.956217)};
\addplot[fig3 mean] coordinates {(0,0.471399) (1,0.960976)};


==> figures/tikz/gen/fig4_moment.tex <==
\fill[fig4 band] (axis cs:0.08,0.518537) rectangle (axis cs:1.14,0.661463);
\draw[fig4 probe] (axis cs:0.08,0.590000) -- (axis cs:1.14,0.590000);
\node[fig4 lab, anchor=south east] at (axis cs:1.14,0.661463) {probe check (same at every $\beta$)};
\addplot[fig4 dots] coordinates {(0.2140,0.475000) (0.2320,0.450000) (0.2500,0.350000) (0.2680,0.325000) (0.2860,0.450000) (0.4640,0.325000) (0.4820,0.425000) (0.5000,0.350000) (0.5180,0.250000) (0.5360,0.475000) (0.9640,0.375000) (0.9820,0.400000) (1.0000,0.350000) (1.0180,0.350000) (1.0360,0.550000)};
\addplot[fig4 mean] coordinates {(0.25,0.410000) +- (0,0.083870) (0.5,0.365000) +- (0,0.108867) (1.0,0.405000) +- (0,0.103885)};


==> figures/tikz/gen/fig4_toto.tex <==
\fill[fig4 band] (axis cs:0.08,0.518983) rectangle (axis cs:1.14,0.791017);
\draw[fig4 probe] (axis cs:0.08,0.655000) -- (axis cs:1.14,0.655000);
\node[fig4 lab, anchor=south east] at (axis cs:1.14,0.791017) {probe check (same at every $\beta$)};
\addplot[fig4 dots] coordinates {(0.2140,0.400000) (0.2320,0.425000) (0.2500,0.500000) (0.2680,0.575000) (0.2860,0.500000) (0.4640,0.425000) (0.4820,0.375000) (0.5000,0.425000) (0.5180,0.475000) (0.5360,0.450000) (0.9640,0.525000) (0.9820,0.275000) (1.0000,0.300000) (1.0180,0.425000) (1.0360,0.425000)};
\addplot[fig4 mean] coordinates {(0.25,0.480000) +- (0,0.086137) (0.5,0.430000) +- (0,0.046042) (1.0,0.390000) +- (0,0.127233)};

